Let Your Camera See for You: A Novel Two-Factor Authentication Method against Real-Time Phishing Attacks

Today, two-factor authentication (2FA) is a widely implemented mechanism to counter phishing attacks. Although much effort has been investigated in 2FA, most 2FA systems are still vulnerable to carefully designed phishing attacks, and some even request special hardware, which limits their wide deployment. Recently, real-time phishing (RTP) has made the situation even worse because an adversary can effortlessly establish a phishing website replicating a target website without any background of the web page design technique. Traditional 2FA can be easily bypassed by such RTP attacks. In this work, we propose a novel 2FA system to counter RTP attacks. The main idea is to request a user to take a photo of the web browser with the domain name in the address bar as the 2nd authentication factor. The web server side extracts the domain name information based on Optical Character Recognition (OCR), and then determines if the user is visiting this website or a fake one, thus defeating the RTP attacks where an adversary must set up a fake website with a different domain. We prototyped our system and evaluated its performance in various environments. The results showed that PhotoAuth is an effective technique with good scalability. We also showed that compared to other 2FA systems, PhotoAuth has several advantages, especially no special hardware or software support is needed on the client side except a phone, making it readily deployable.

==> optimization.tex <==

\subsection{Performance Optimization Module}
\label{sec:optimization}
%new add%%%%%%%%%%%%%
In the real-world cases, users who have been hijacked by the RTP attacks should be the minority among all users of a system. That is, most user logins (authentication requests) are normal. Now, if PhotoAuth requires all users to take photos of their browsers for authentication all the time, that will incur much burden for the server. Below we present several strategies to optimize for performance.

%In the real-world cases, users who have been hijacked by the RTP attacks should be the minority among all users of a system. That is, most user logins (authentication requests) are normal. Now, if PhotoAuth requires all users to take photos of their browsers for authentication, that will incur much burden for the server. Below we present several strategies to optimize for performance, with slightly weaker security guarantee, compared to the case running PhotoAuth for every login request (or other security critical requests that require additional authentication such as money transfer in bank websites). 

Figure \ref{fig:system_optimization} shows the flowchart for our performance optimization mechanisms. 
Take Microsoft as an example again. When the Microsoft web server gets Bob's authentication request (the top rectangle symbol in the figure), it first checks the cookie of the request to see whether Bob has been authenticated previously. If yes, the server knows this is an ongoing session, so it authorizes the authentication request directly (The flow goes to the right branch in Figure \ref{fig:system_optimization} ). Requests with invalid cookies may result in the ``400 Bad Request" error (we ignore this case in the figure).  


\begin{figure}[h]
\centering
\includegraphics[scale=0.35]{image/system_optimization.pdf}
\caption{System Optimization}
\label{fig:system_optimization}
\end{figure}

If the request has no cookie, it is a new session. In this case, the server checks its record for Bob's preferred 2FA method. 
%(Figure \ref{fig:system_optimization} goes to the left branch at the first diamond area and enter to the second diamond). 
%new add%%%%%
If the preference is to receive an SMS/Push message (preference email has same flow), he will receive an SMS/Push message through his phone, which contains a short link like microsoft.com/c/689527. Here the 6-digit number is Bob's session id. 
Microsoft server obtains the cookie of Bob's authentication request on Bob's phone when Bob clicks the short link on his phone. It then compares this cookie with the one in the previous authentication request. 


%If the preference is to receive an SMS/Push message, he will receive an SMS/Push message through his phone, which contains a short link like microsoft.com/c/689527. Here the 6-digit number is Bob's session id. 
%Microsoft server obtains the IP address of Bob's phone when Bob clicks the short link on his phone. It then compares this IP address with the one in the previous authentication request.

%(Figure \ref{fig:system_optimization} the diamond of the right branch of the second diamond). 

%new add%%%%%
%If they are the same, then it is the case where Bob is using the same browser to login and to handle SMS/Push short link, it is a legitimate request from Bob. Hence, it will be authorized by the server. SMS/Push messages must be received by phone. That also means Bob is using phone browser to login and click the short link. Otherwise, no matter that it is because Bob opens the short link in a different browser or there exists a RTP attack, the server proceeds with PhotoAuth 2FA. If the cookie is different, it has three cases under RTP phishing, PC sends login but clicks the short link on the phone, the phone sends login but clicks the short link with another phone browser. PhotoAuth can handle the first two cases. For the third one, the server can pop up a message to remind the user that the login request is from the phone, the user should use the same phone browser to open the short link. 
%With the above performance optimization, only a small percent of users need to go through the PhotoAuth 2FA. 


%If they are the same, then it is the case where Bob's computer and phone are connected to the same network behind the NAT, e.g., in a typical home network. 

%It is very hard for the adversary to use Bob's network IP to send an authentication request. 
%Because a pure phishing attack cannot establish a proxy with a victim's IP in the victim's device. 
%Therefore, the server will authorize the authentication request. 

%If the two IP addresses are different, there are multiple possible causes. First, Bob's phone and computer are connected to two different networks. For example, Bob's phone uses a 4G cellular network but his computer uses WiFi. 
%Second, Bob's phone and computer belong to two different subnets that are both publicly visible. For example, in a university setting, Bob's computer has a fixed IP address belonging to the computer science department, but his phone joins the university's WiFi network. The third case is that Bob's computer uses a remote proxy or a VPN to login, while his phone uses a cellular network or WiFi. The fourth case is that Bob is under the RTP attack, where the adversary uses his own computer in a different network (or in the same network if the adversary is co-located with the victim) to login as Bob. There could be other special cases. 

%No matter which case it is, as long as the IP addresses are different, the server requires Bob take a photo of his browser to verify the domain name, because it does not know exactly which case it is. While this looks very strict, as some legitimate requests may require PhotoAuth 2FA, it is for stronger security. Certainly, in practice a system may choose to go for better performance based on some heuristics, as commonly done by the industry. For example, Google uses IP geolocation to identify abnormal logins and alerts users through emails. 
%If the website owner accepts the risk of co-location RTP attacks, where the adversary is (or has compromised a computer) in the same network as the victim,  or he is in the same city as the victim, it may approve the case as long as two IP addresses are from the same network or from the same city (based on IP geolocation). Note that the server may also remember the list of most frequently used IP address of each user, so that PhotoAuth 2FA is not necessary if a request is from the same IP. After all, the system may decide what is the best choice based on the importance of its operations.       

%If Bob's preference is to invoke 2FA via email, Bob will receive an email that contains the same short link. Again, the server will collect Bob's session cookie and IP after Bob clicks the short link. If the enclosed cookie is  valid, which indicates that Bob is using the same browser to login and to handle emails, it is a legitimate request from Bob. Hence, it will be authorized by the server. Otherwise, no matter that it is because Bob opens the email short link in a different browser or there exists a RTP attack, similar to the way SMS/push message is handled, if they have the same IP, the server authorizes the authentication request; otherwise, the server proceeds with PhotoAuth 2FA. 


==> scratch.tex <==

\subsection{Optimization Module}
In the real-world cases, users who have been hijacked by the RTP attacks should be the minority among all users of a system. That is, most user logins (authentication requests) are normal. Now, if PhotoAuth requires all users to take photos of their browsers to finish authentication, that will incur too much extra burden for users. Below we present several strategies to optimize for performance, with slightly weaker security guarantee, compared to the case running PhotoAuth for every login (or other security critical requests that require additional authentication such as money transfer in bank websites). 

Figure \ref{fig:system_optimization} shows the flowchart for our performance optimization mechanisms. 
Take Microsoft as an example again. When the Microsoft web server gets Bob's authentication request (the top rectangle symbol in the figure), it first checks the cookie of the request to see whether Bob has been authenticated previously. If yes, the server knows this is an ongoing session, so it authorizes the authentication request directly (The flow goes to the right branch in Figure \ref{fig:system_optimization} ). Requests with invalid cookies may result in the ``400 Bad Request" error (we ignore this case in the figure).  

If the request has no cookie, it is a new session. In this case, the server checks its record for Bob's preferred 2FA method. 
%(Figure \ref{fig:system_optimization} goes to the left branch at the first diamond area and enter to the second diamond). 
If the preference is to receive an SMS/Push message, he will receive an SMS/Push message through his phone, which contains a short link like microsoft.com/c/689527. Here the 6-digit number is Bob's session id. 
Microsoft server obtains the IP address of Bob's phone when Bob clicks the short link on his phone. It then compares this IP address with the one in the previous authentication request. 
%(Figure \ref{fig:system_optimization} the diamond of the right branch of the second diamond). 
If they are the same, then it is the case where Bob's computer and phone are connected to the same network behind the NAT, e.g., in a typical home network. %It is very hard for the adversary to use Bob's network IP to send an authentication request. 
%Because a pure phishing attack cannot establish a proxy with a victim's IP in the victim's device. 
Therefore, the server will authorize the authentication request. 

If the two IP addresses are different, there are multiple possible causes. First, Bob's phone and computer are connected to two different networks. For example, Bob's phone uses a 4G cellular network but his computer uses WiFi. 
Second, Bob's phone and computer belong to two different subnets that are both publicly visible. For example, in a university setting, Bob's computer has a fixed IP address belonging to the computer science department, but his phone joins the university's WiFi network. The third case is that Bob's computer uses a remote proxy or a VPN to login, while his phone uses a cellular network or WiFi. The fourth case is that Bob is under the RTP attack, where the adversary uses his own computer in a different network (or in the same network if the adversary is co-located with the victim) to login as Bob. There could be other special cases. 

No matter which case it is, as long as the IP addresses are different,  Figure~\ref{Sec:Optimization_Module} shows that the server requires Bob take a photo of his browser to verify the domain name, because it does not know exactly which case it is. While this looks very strict, as some legitimate requests may require PhotoAuth 2FA, it is for stronger security. Certainly, in practice a system may choose to go for better performance based on some heuristics, as commonly done by the industry. For example, Google uses IP geolocation to identify abnormal logins and alerts users through emails. 
If the website owner accepts the risk of co-location RTP attacks, where the adversary is (or has compromised a computer) in the same network as the victim,  Or he is in the same city as the victim, it may approve the case as long as two IP addresses are from the same network or from the same city (based on IP geolocation). Note that the server may also remember the list of most frequently used IP address of each user, so that no PhotoAuth 2FA is necessary if a request is from the same IP. After all, the system may decide what is the best choice based on the importance of its operations.       

If Bob's preference is to invoke 2FA via email, Bob will receive an email that contains the same short link. Again, the server will collect Bob's session cookie and IP after Bob clicks the short link. If the enclosed cookie is  valid, which indicates that Bob is using the same browser to login and to handle emails, it is a legitimate request from Bob. Hence, it will be authorized by the server. Otherwise, no matter that it is because Bob opens the email short link in a different browser or there exists a RTP attack, similar to the way SMS/push message is handled, if they have the same IP, the server authorizes the authentication request; otherwise, the server proceeds with PhotoAuth 2FA. 
With the above performance optimization, only a small percent of users need to go through the PhotoAuth 2FA. 

==> userstudy.tex <==
\subsection{A Preliminary User Study}

\begin{figure}[htbp!]
    \centering
    %   \begin{subfigure}[b]{0.3\textwidth}
    %     \includegraphics[width=\textwidth]{image/guide_video_screenshot.png}
    %       \caption{The screenshot of PhotoAuth guide video with subtitles.}
    %       \label{fig:guide_video_screenshot}
    %   \end{subfigure}
    %   \hfill
    
    %   \begin{subfigure}[b]{0.3\textwidth}
    %     \includegraphics[width=\textwidth]{image/survey_question.png}
    %       \caption{User study survey question}
    %       \label{fig:survey_question}
    %   \end{subfigure}
    %   \hfill
    
      \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{image/background_of_2fa.png}
          \caption{User's prior experience with 2FA}
          \label{fig:background_of_2fa}
      \end{subfigure}
      \hfill

      \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{image/rate_of_photoauth.png}
          \caption{User's evaluation of PhotoAuth}
           \label{fig:rate_of_photoauth}
      \end{subfigure}
      
\caption{User study}
\label{fig:user_study}
\end{figure}

A comprehensive user study is intractable at this stage of our research for various reasons. Ideally, we may set up a working system for each participant to 
have the first-hand experience. However, in this case a user's opinion about our system may be greatly influenced by the details of our implementation, such as the performance of the system at the specific use time, the design of the web GUI, etc. Indeed, in our prototype we use a free online service for delivering SMS messages to mobile phones. Such a service is not stable (in one case it took five minutes to deliver) and occasionally SMS messages may even be blocked by cellular service providers. Too many differences between our prototype system and a real-world commercial system that would deploy PhotoAuth will prevent us from obtaining meaningful user feedback.    

As such, in this stage, we only conduct a preliminary user study regarding the overall workflow of the system. 
We made a short live tutorial video (around 1 minute 30 seconds) to demonstrate the 2FA process step-by-step. It starts with the username/password login page (Figure~\ref{fig:website_interface}, followed by several UIs in both PC and phone (including those UIs in Figure~\ref{fig:one_hash_represent}). Each UI in the video has one or two sentences subtitle (instead of voice) to explain the high-level idea or procedure. As a result, users do not know exactly how our technique works through this video tutorial. We choose to do so because our study cares more about the overall usability of the system for ordinary users. After that, a user is asked to answer a questionnaire with three simple questions, as shown in Figure~\ref{fig:survey_question}.   
We obtained the IRB approval from our university for this anonymous user study, which does not ask and collect any personal information from participants.

We tried to recruit participants from our personal social networks with various  technical background. As the survey was anonymous and the participation was totally voluntary, we do not know who submitted the survey and do not know the demographic information of the participants. 
In the end, we collected 33 survey feedback.   

%We did an anonymous user study survey on PhotoAuth. We provide guide video, as figure~\ref{fig:guide_video_screenshot} shows, for users to show the whole workflow of PhotoAuth. After users watch the video, they can test and then fill out the questionnaire as figure~\ref{fig:survey_question} shows. We expect that even users have no background of computers, they can still correctly operate PhotoAuth to finish authentication. So most participants have no computer background. 
%Our questions have two types that are multi-choice and short-answer questions. Totally 33 persons participate in our survey. To protect users' privacy. We didn't collect the private data of users like names.

Figure~\ref{fig:background_of_2fa} shows that most participators have used a 2FA system before, with SMS and Duo Mobile being the most popular, so they have the basic understanding of 2FA. Figure~\ref{fig:rate_of_photoauth} shows that slightly over 50\% of users considered PhotoAuth ``as convenient as the 2FA system I have used before", 24.2\% users rated it ``a little bit more difficult than the 2FA system I have used before but intuitive to use'', 21.2\% of users rated ``a little barrier at the first time, but it becomes intuitive to use afterward''. Most users held a positive attitude regarding the usability of PhotoAuth. 

Clearly, this is only a preliminary user study. In our future work, we will consider designing and conducting a more comprehensive user study.  


